FLEX: Expert-level False-Less EXecution Metric for Reliable Text-to-SQL Benchmark

Text-to-SQL systems have become crucial for translating natural language into SQL queries in various industries, enabling non-technical users to perform complex data operations. The need for accurate evaluation methods has increased as these systems have grown more sophisticated. However, the Execution Accuracy (EX), the most prevalent evaluation metric, still shows many false positives and negatives. Thus, this paper introduces FLEX (False-Less EXecution), a novel approach to evaluating text-to-SQL systems using large language models (LLMs) to emulate human expert-level evaluation of SQL queries. Our metric improves agreement with human experts (from 62 to 87.04 in Cohen's kappa) with comprehensive context and sophisticated criteria. Our extensive experiments yield several key insights: (1) Models' performance increases by over 2.6 points on average, substantially affecting rankings on Spider and BIRD benchmarks; (2) The underestimation of models in EX primarily stems from annotation quality issues; and (3) Model performance on particularly challenging questions tends to be overestimated. This work contributes to a more accurate and nuanced evaluation of text-to-SQL systems, potentially reshaping our understanding of state-of-the-art performance in this field.

==> 04_method_old.tex <==

\section{Method}
\label{sec:method}


% - Schema(2): 3, 28
% - Condition (4): 28, 31, 59, 74
% - Abused Clauses (1): 66
% - Null Aggregation (2): 72, 73
% - Multiple Rows (1): 49


% Overused Column (5) = 6, 48, 58, 70, 90
% Column Order (6): 17, 29, 31, 43, 89, 96
% Representation (2): 16, 35
% Others (2): 26, 86
% Incorrect GT (2): 59, 98



This section outlines \ours~for evaluating Text-to-SQL models using LLMs, addressing the limitations mentioned earlier. Our approach consists of three key steps: query generation, LLM-based judgment, and comprehensive evaluation. 

\subsection{Step 1: Query Generation and Execution}
\hist{EX metric 위에서 동작하는 방식이라면 (execution result 와 ground truth 를 비교한 후에 그에 따라서 검사하는게 달라지는 방식이라면), step 1 을 생략해도 될 것 같습니다. metric 에 대한 연구인 만큼, metric 에 입력으로 들어가는게 무엇인지만 명확히 define 하면 될 것 같습니다. (그 입력들을 어떻게 만드는지는 굳이 설명하지 않고)}
First, using the database schema and supplementary information, the text-to-SQL model generates a SQL query from a natural language question. The BIRD dataset provides a schema description and supplementary information for each question.
For each text-to-SQL sample, we execute the generated and ground truth queries on the target database. This step is crucial to retrieving the execution results, which are part of the input to the LLM judgment. 

\subsection{Step 2: LLM Judgment}
\label{sec:sec_judgement}
After execution, the LLM is asked to evaluate using the sophisticated designed prompt.
\hist{Additional Context 랑 Customized Criteria 가 어떤 맥락에서 나오는 건지 잘 모르겠습니다. prompt 가 아래 2가지를 특별히 고려해서 작성되었다는 걸까요?}

\textbf{1) Additional Context:} \ours~provides the natural language question, the generated query's execution result, external knowledge, a ground truth query with its execution result, and the SQL Database schema with natural language description. \hist{FLEX 는 metric 인데 입력으로 들어갈 만한 내용들을 provides 한다는게 어색한 듯 합니다. takes 같은걸 의도한걸까요?}
\ours~does not provide execution results when the generated query produces the equivalent results as ground truth. The equivalent execution results demonstrate a negative influence on the evaluation of false positives. 

\textbf{2) Customized Criteria:} Based on the error cases in a human study \hist{앞에서 다뤄진 내용이라면 reference 가 있으면 좋을 듯}, criteria are customized according to whether the execution result is the same. We specify the following categorized error cases for accurate evaluation.
Actual prompts are described in appendix~\ref{sec:appendix_prompt}.

\hist{4.2.1 이랑 4.2.2 첫 문장 읽고 든 생각인데, executul result 와 ground truth 의 매칭 여부에 따라 분기가 나뉜다는걸 명시하고 넘어가야 이해가 잘 될 것 같습니다. 비슷한 맥락에서, Criteria for False Positives 보다는 False Positive Check 라거나... EM (GT, Execution) 인 경우에 무엇을 체크하는지... 를 나타낼 수 있는 subsubsection title 이면 좋을 것 같습니다.}

\subsubsection{Criteria for False Positives}
\label{sec:method_fn}

For the same execution result, the LLM analyzes the difference between the two queries to detect false positives. 
It infers the impact of diverse scenarios in the current schema, causing an incorrect result for the user's question when the database rows are updated. 
The LLM judges the following cases as incorrect:
\begin{itemize}[noitemsep,topsep=5pt,parsep=2pt,partopsep=0pt,leftmargin=*]
    \item Incorrect Schema Linking: Ensure that tables and columns in the generated query align with the question and the provided schema.
    \item Incorrect Filtering Conditions: Verify that the query correctly filters data based on the given conditions, ensuring the WHERE clause is used appropriately to match the expected results.
    \item Missing Handling of the Nullable Column: Check if the query correctly handles nullable columns in aggregation functions (SUM, COUNT, AVG) of WHERE clauses, as improper handling can lead to unexpected results.
    \item Missing Handling of Multiple Rows: Determine if the query correctly accounts for scenarios where multiple rows might satisfy the condition, potentially leading to incorrect answers.
    \item Multiple Answers Available: The question is ambiguous and can be semantically represented by multiple queries.
    \item Clause Abusing: Evaluate if SQL clauses like GROUP BY, HAVING, ORDER BY, and DISTINCT are used unnecessarily, which could produce incorrect results.
\end{itemize}

\subsubsection{Criteria for False Negatives}
For the generated queries producing different execution results, the LLM not only evaluates logical correctness using section~\ref{sec:method_fn} criteria but also considers whether output structure differences are acceptable.
When the question does not specify, and the query's result contains sufficient content to answer the question, the following cases are allowed:
\begin{itemize}[noitemsep,topsep=5pt,parsep=2pt,partopsep=0pt,leftmargin=*]
    \item Different output structures in column/row order, extra or missing columns.
    \item Differences in the representation of values, such as formatting (percentile, YES/NO) or data types for readability.
    \item Due to ambiguous questions interpretable to multiple queries, the generated query's execution may differ from the ground truth.
    \item The ground truth query is incorrect, but the generated query is correct.
\end{itemize}


\subsection{Step 3: Evaluation Summary}

\hist{너무 좋은 기능?이기는 한데, 이게 metric 으로 엮일 수 있는지 좀 애매한 것 같습니다. experiments 로 옮기고 해당 report 생성에 대한 기능은 open-source로 공개했다고 하는게 더 자연스럽지 않을까 싶네요.}
We generate a comprehensive evaluation report after obtaining judgments for all generated queries in a dataset.
This report includes an overall accuracy score, a breakdown of error types, and detailed explanations for each incorrect query. 
The LLM is prompted to categorize the error case based on its judgment and other contextual information.
Judgments are categorized according to the criteria described in the previous subsection, and complex errors can belong to more than one category.
Researchers can utilize this evaluation report to identify systematic errors in their text-to-SQL models and guide future improvements. 



==> 07_discussion.tex <==
\section{Discussion}
% \hist{태양: discussion 써봤는데 분량이 조금 많네요.}
% Our observations using \ours~underscore the need for a paradigm shift in text-to-SQL system evaluation and development. The discrepancy between EX and \ours~scores, especially for complex questions, suggests current models excel at simple patterns but struggle with intricate database semantics. This highlights the need for more challenging datasets to assess and improve models' comprehension abilities.
% Our analysis reveals performance variations across model types (proprietary, open PLMs, open SFT), suggesting current evaluation methods may reward superficial pattern matching over genuine database comprehension. This emphasizes the need for more robust evaluation methods and datasets.
% Many false negatives stem from ambiguous questions and incorrect ground truths, underscoring the need for more rigorous benchmark creation. Future benchmarks should incorporate multiple ground truth queries, unambiguous questions, and precise output specifications.
% The success of \ours~in emulating human expert evaluation opens new possibilities for AI-assisted assessment while raising questions about potential bias amplification. Future work should focus on aligning \ours~with human expert judgments and mitigating evaluation biases.
% In conclusion, \ours~provides a more accurate evaluation metric and catalyzes rethinking our approach to text-to-SQL tasks, challenging us to develop more sophisticated models and create more robust benchmarks. By addressing these challenges, we can push the boundaries of text-to-SQL systems, leading to more reliable and capable database interfaces in the future.
% \hist{희규:}
\ours~demonstrates promising results in LLM-based text-to-SQL evaluation, yet it faces limitations primarily due to insufficient contextual information. 
To enhance the accuracy of LLM-based evaluations, the future text-to-SQL benchmarks should incorporate multiple ground truth queries per question, more comprehensive schema details, and additional context regarding database relationships and constraints.
GPT-4o exhibits potential biases in false positive evaluations, which diminishes human-AI agreement. 
To address this issue in the future, we suggest implementing advanced prompting techniques such as Self-Consistency~\cite{wang2022selfconsistency} or employing an ensemble of LLM judges. 
These strategies aim to mitigate individual model biases and enhance LLM-based evaluations' overall reliability and fairness. 
Continuous fine-tuning of the evaluation process based on human expert feedback is crucial for maintaining and improving the system's performance over time.

\ours~uncovered a substantial performance gap between proprietary models like GPT-4 and open alternatives such as CodeS~\cite{li2024codes} and RESDSQL~\cite{li2023resdsqldecouplingschemalinking}. 
While proprietary models exhibit superior performance, their use in real-world text-to-SQL applications raises concerns, particularly regarding data leakage~\cite{Writingsofrach_2024}. 
\ours~could be employed for diverse and high-quality data augmentation, potentially enhancing open SFT models.
This will narrow the performance disparity between open-source and proprietary models and advance the field of text-to-SQL translation.

% Our observations using \ours~suggest several directions for improving text-to-SQL benchmarks and models.
% Both human experts and language models (LLMs) require additional context for more accurate evaluations. 
% The additional context is particularly important when dealing with dirty databases like BIRD, which mirror real-world scenarios with redundant columns across multiple tables and unclear constraints. 
% To address this, we propose including the following components during the annotation process: multiple ground truth queries implemented in various ways, unambiguous questions, clear output structure specifications, and criteria for correct answers. 
% \ours~revealed a significant performance advantage of proprietary models like GPT-4 over open-source models such as CodeS~\cite{li2024codes} and RESDSQL~\cite{li2023resdsqldecouplingschemalinking}.
% However, the reliance on proprietary LLMs for text-to-SQL tasks presents challenges for real-world applications, particularly due to concerns about data leakage~\cite{Writingsofrach_2024}.
% This performance disparity highlights the need for continued research and development of open-source alternatives. The goal is to create models that can offer comparable performance while addressing data privacy and security concerns, making them more suitable for widespread adoption in various industries and applications.
%%% 위에는 원본

% As illustrated in Fig~\ref{fig:cat_top10_fp} and \ref{fig:cat_top10_tn}, the primary sources of error for false positives and true negatives are incorrect schema linking, incorrect filtering conditions, and missing handling of multiple rows.
% Interestingly, we observed a notable difference in the proportion of `Other' errors between false positives and true negatives. 
% While the `Other' category constituted a relatively small portion of false positives, it represented a significant proportion of true negatives. 
% This suggests that true negatives often involve more complex or logical errors that do not fall neatly into our predefined categories.

% The top ten Spider-dev models demonstrate similar false negatives and false positives patterns. 
% Since top models in Spider demonstrate approximately 90\% accuracy of \ours, average counts of false negatives were less than 20 questions.
% However, the most common cause of true negatives is incorrect filtering conditions, which have a noticeable gap compared to other categories.
% This suggests that researchers should study improving the accuracy of Spider's filtering conditions to match the user's question.

==> bak.tex <==
% EM and EX do not consider ambiguous questions that can be interpretable to multiple queries and incorrectly annotated ground truths. 




% \input{table/pre/simple_error_cases}


% To illustrate these limitations, consider the following examples illustrated in the table~\ref{tab:tab_fp_fn_example}:
% Conversely, the false negative example is semantically correct but produces the additional column `score.' EX considers this minor difference an incorrect query. The main reason is that the question does not specify the output columns, and the ground truth of the benchmark is inconsistent. 
% In EX, output representation differences for reader convenience are considered incorrect, such as converting rate to percentage and answering yes/no rather than true/false to the question of existence.

% Annotation quality is another major issue in the text-to-SQL benchmarks. 


% This section investigates the limitations of conventional text-to-SQL evaluation metrics and LLM-based text-to-SQL evaluation. 
% In our analysis, they still need to improve to achieve expert-level text-to-SQL evaluation.

% The EX, which only compares execution results, cannot detect this logical error.


% Due to these limitations, in our human-LLM agreement evaluation, \llmsqlsolver using GPT-4o yields 52.78 score of Cohen's kappa, significantly lower than EX~(62) and our \ours~(78.17). 


% This result strongly demonstrates that \ours is much more suitable than \llmsqlsolver to evaluate text-to-SQL systems.


% The limitations of the EX metric and the insights from our human evaluation study strongly advocate the introduction of a new evaluation paradigm.
% This paradigm should incorporate a more semantic assessment of SQL query correctness, allowing for a more accurate and human-expert-level evaluation of text-to-SQL systems.
% However, scaling human evaluation is challenging due to its time-intensive nature and high cost. 
% Recent works have explored using LLMs to assess generation tasks. 
% Approaches like AlpacaEval~\cite{alpaca_eval} and MT-Bench~\cite{zheng2023judgingllmasajudgemtbenchchatbot} have demonstrated the potential of LLMs in evaluating generated text and multi-turn interactions. 
% However, these methods are not specifically tailored to the unique challenges of SQL query evaluation, such as understanding database schemas and query logic.



% To the best of our knowledge, our work is the first to propose an LLM-based evaluation framework specifically designed for human-expert-level text-to-SQL evaluation. 
% Unlike previous approaches that rely solely on traditional metrics or apply general-purpose LLM evaluation techniques, our method integrates domain-specific SQL knowledge with LLMs' reasoning capabilities.
% This novel approach enables a more comprehensive assessment of semantic correctness and query logic beyond simple exact matching of SQL queries or execution results. 
% By addressing the limitations of existing evaluation methods, our framework provides deeper insights into the quality and correctness of generated SQL queries, considering factors such as schema understanding and query complexity. 
% This approach, by offering a more semantically accurate evaluation methodology, has the potential to drive significant advancements in text-to-SQL research.




% The consensus between human judgments are set to ground truths, and other LLM judgments and EX are predictions. 
% Cohen's kappa and accuracy are utilized to measure human agreement between experts. \hist{이 문장의 앞뒤는 implementation detail 인데, 이 문장은 evaluation protocol 에 대한 내용이라 중간에 들어가기가 살짝 어색한 것 같습니다.}
% In Prometheus-2, we converted our LLM prompt to the absolute judge template. 
% Prometheus-2 yields scores between one and five; the higher the score, the more correct the generated query.
% We considered scores four and five correct, demonstrating the highest agreement.
% \hist{In Prometheus-2, we converted our judge template to the absolute one. As Prometheus-2 generates scores ranging from one to five, where the higher score means the more accurate query, we deemed scores of four and five as correct, indicating the highest level of agreement.}

% \input{table/exp1/true_positive_v2}
% \input{table/exp1/true_positives}

% A notable example is demonstrated in table~\ref{tab:tab_confusable_true_positive} that the ground truth joins the unnecessary ``schools" table, but the prediction query does not. Although this difference does not affect the execution result, it could be confused as a schema linking error. GPT-4o-mini, Gemini-1.5-flash, and Llama-3.1-70B-Instruct judged that the prediction was wrong, but others judged it as correct. These observations support using LLMs, particularly advanced models like GPT-4o, as influential judges for text-to-SQL evaluation. The high agreement with human judgments suggests that this approach can provide a more accurate and nuanced assessment of SQL query correctness than traditional metrics.

% The most crucial factor, criteria, supports the underperforming LLM-SQL-Solver, only providing schema and queries, even with the same base LLM, GPT-4o.

% However, including execution results influences performance according to the equivalence of the generated query's execution result to ground truth. Equivalent execution results hinder the false positive evaluation even if the generated query has the incorrect logic. Conversely, in the not equivalent set, including the execution result benefits the false negative evaluation because the LLM directly compares the minor differences. The most crucial factor, criteria, supports the underperforming LLM-SQL-Solver, only providing schema and queries, even with the same base LLM, GPT-4o.

% Our study reveals distinct patterns of two benchmarks across question difficulty levels. 
% The models show consistent performance improvement in \ours~ compared to the EX metric in Spider, while this trend is not observed in BIRD. 
% This discrepancy can be elucidated through an analysis of error type ratios. 
% In Spider, as illustrated in Fig~\ref{fig:hardness-flex-ex-fp-fn-line}, both false positive (FP) and false negative (FN) ratios increase consistently with question difficulty. 
% However, the FN ratios consistently exceed FP ratios, resulting in FLEX outperforming EX across all difficulty levels. 
% Conversely, BIRD exhibits a decrease in FLEX performance gain as question difficulty increases. 
% This trend is due to fluctuating FN ratios and increasing FP ratios as questions become more difficult.

% Moreover, we observed contrasting patterns in difficult questions between the two benchmarks. 
% In Spider, the models' performance appears to be underestimated in the EX metric, particularly for more difficult questions. 
% Specifically, easy and medium questions demonstrate minimal improvement with the \ours~metric due to already high EX scores (88.08 for easy and 78.93 for medium). 
% However, hard and extra hard questions, which exhibit lower EX scores (64.14 for hard and 49.74 for extra hard), show significant gains due to high false negatives. 
% This difference leads to a distinct underestimation of performance on difficult questions when using the traditional EX metric.
% Conversely, in BIRD, we found that the models' performance is overestimated for difficult questions when using the EX metric. Simple and moderate questions show performance gains with \ours, while challenging questions exhibit a steep decrease in performance.


% \textbf{Dataset:} In BIRD, we randomly sampled 200 query pairs generated by TA-ACL~\cite{qu2024generationalignitnovel} and SuperSQL~\cite{li2024dawn}, evenly split between queries showing the same result as ground truth (Equivalent set) and those with different results (Not equivalent set). 

% \textbf{Human Annotation:} Three human experts with over three years of SQL experience independently evaluated these queries, and samples with different annotations were annotated by consensus. Before consensus, inter-annotator agreement was measured using Fleiss' kappa, yielding a value of 86.7, indicating almost perfect agreement.

% \textbf{Metric:} We employed Cohen's kappa and accuracy score to measure agreement between human experts and EX.

% \textbf{Human Experts vs. EX:} The agreement between human consensus and EX measured using Cohen's kappa yielded 62.0, indicating substantial agreement but much room for improvement. 
% Human annotators found 21 false positives in the not equivalent set. 
% They found 17 false negatives in the equivalent set. 
% These findings raise concerns about the current text-to-SQL leaderboard's reliability and underscores the need for a new method that aligns more closely with human judgment, considering semantic correctness and offering a more granular assessment of query accuracy. 
% Real instances are described in appendix~\ref{sec:appendix_errors}.


% In \prometheustwo, we designed two types of rubric templates\footnote{Detailed prompts are provided in Appendix~\ref{sec:appendix_prompt_prometheus}.}:
% \begin{itemize}
%     \item Ambiguous Template (A): Describes general criteria such as "How accurately does the model translate natural language queries into correct and efficient SQL queries?"
%     \item Customized Template (C): Utilizes different templates for each evaluation set, describing specific criteria. 
% \end{itemize}

==> image/method/prompt_strict.tex <==

\begin{figure}[h]
\centering
\begin{verbatim}

You should evaluate a SQL query that translates a natural language question. You should compare the prediction query with the ground truth query to evaluate whether the given table schema can always produce the same results. For example, when rows are added or deleted from an existing table, the prediction query should always produce the same results as the ground truth query.

You can always achieve the same result even if the two queries use different tables or columns. Therefore, you should carefully and accurately judge by referring to the given schema and description information. Different approaches can be used to answer a user's question, and sometimes different results can occur. For example, you can use subquery to get the maximum value, or you can use a combination of order by and limit. This can lead to different results, but also evaluate whether the query matches the question.

Judge Rules
1. Do not consider clarity, efficiency or readability in your evaluation.
2. Answer using following format:
**Analysis**
// Write your step-by-step feedback here
**Decision**
```yaml
equivalence: str # equal or not_equal
correct: boolean # True if prediction query is correct, False if not
```
\end{verbatim}
\caption{Example of false positive queries.}
\label{fig:false_positive}
\end{figure}

==> prompt/prometheus_ambiguous.tex <==
Criteria: How accurately does the model translate natural language queries into correct and efficient SQL queries?
Score 1: The generated SQL query is completely incorrect and does not address the user's request.
Score 2: The SQL query partially addresses the user's request but contains significant errors or omissions.
Score 3: The SQL query mostly addresses the user's request with minor errors or inefficiencies.
Score 4: The SQL query correctly addresses the user's request with only trivial issues, if any.
Score 5: The SQL query perfectly translates the user's request into an accurate and efficient SQL statement.

==> table/exp1/ablation.tex <==
% \usepackage{tabularray}
% \begin{table}[!h]
% \centering
% \caption{A result of the ablation study. Including execution results affects performance, depending on whether the generated query has equivalent results to the ground truth. Criteria is the most crucial component of the evaluation.}
% \label{tab:tab_flex_ablation}
% \adjustbox{max width=\linewidth}{
% \begin{tblr}{
%   column{even} = {c},
%   column{3} = {c},
%   column{5} = {c},
%   hline{1,8} = {-}{0.08em},
%   hline{2} = {-}{0.05em},
%   hline{3} = {-}{dashed},
% }
% \textbf{Model}           & \textbf{Kappa} & \textbf{Acc.}  & \textbf{EQ} & \textbf{NEQ} \\
% \textbf{FLEX (base)}     & \textbf{87.04}          & \textbf{93.5}          & \textbf{88}          & \textbf{99}           \\
% \textit{Always w/o Exec.}   & \underline{82.06} & \underline{91.0} & \textbf{88} & 94           \\
% \textit{Always w/ Exec.}    & 81.08          & 90.5          & 82          & \textbf{99}  \\
% \textit{w/o Question}    & 80.10          & 90.0          & \underline{84}          & 96           \\
% \textit{w/o External KG} & 79.09          & 89.5          & 82          & \underline{97}           \\
% \textit{w/o Criteria}    & 74.08          & 87.0          & 81          & 93           
% \end{tblr}
% }
% \end{table}
\begin{table}[!h]
\centering
\caption{A result of the ablation study. \emph{NEQ-only} denotes that factor is provided to LLM only when $R_{gt}(x) \neq R_{gen}(x)$}
\label{tab:tab_flex_ablation}
\adjustbox{max width=\linewidth}{

\begin{tabular}{cccc;{1pt/1pt}cc|cccc} 
\hline
$\mathbf{X}$ & $\mathbf{K}$ & $\mathbf{C}$ & \sqlgt   & \exgt    & \exgen                              & \textbf{Kappa} & \textbf{Acc}  & \textbf{EQ} & \textbf{NEQ}  \\ 
\hline
\multicolumn{6}{c|}{$\mathbb{C}_{FLEX}$}                                                                            & \textbf{87.04} & \textbf{93.5} & \textbf{88} & \textbf{99}   \\ 
\hdashline
$\circ$      & $\circ$      & $\circ$      & $\circ$  & $\times$ & $\times$                            & \uline{82.06}  & \uline{91.0}  & \textbf{88} & 94            \\ 
\cdashline{5-6}[1pt/1pt]
$\circ$      & $\circ$      & $\circ$      & $\circ$  & \multicolumn{2}{c|}{\multirow{4}{*}{NEQ-only}} & 81.08          & 90.5          & 82          & \textbf{99}   \\
$\times$     & $\circ$      & $\circ$      & $\circ$  & \multicolumn{2}{c|}{}                          & 80.10          & 90.0          & \uline{84}  & 96            \\
$\circ$      & $\times$     & $\circ$      & $\circ$  & \multicolumn{2}{c|}{}                          & 79.09          & 89.5          & 82          & \uline{97}    \\
$\circ$      & $\circ$      & $\times$     & $\circ$  & \multicolumn{2}{c|}{}                          & 74.08          & 87.0          & 81          & 93            \\ 
\cdashline{5-6}[1pt/1pt]
$\circ$      & $\circ$      & $\circ$      & $\times$ & $\times$ & NEQ-only                            & 29.36          & 64.0          & 72          & 56            \\
\hline
\end{tabular}

}
\end{table}

% \begin{table}[!h]
%   \centering
%   \caption{A result of the ablation study. GT denotes \sqlgt~and \exgt.}
%   \label{tab:tab_flex_ablation}
%   \adjustbox{max width=\linewidth}{
%   \begin{tblr}{
%     cells = {c},
%     vline{3,7} = {-}{},
%     hline{1-3,10} = {-}{},
%     hline{4} = {-}{dashed},
%     rowsep = 0.5pt,
%   }
%   \SetCell[c=2]{c} $\mathbf{R^*(x)}$ & & \SetCell[r=2]{c} $\mathbf{X}$ & \SetCell[r=2]{c} $\mathbf{K}$ & \SetCell[r=2]{c} $\mathbf{C}$ & \SetCell[r=2]{c} \textbf{GT} & \SetCell[r=2]{c} \textbf{Kappa} & \SetCell[r=2]{c} \textbf{Acc} & \SetCell[r=2]{c} \textbf{EQ} & \SetCell[r=2]{c} \textbf{NEQ} \\
%   \textbf{$\mathbb{C}_{EQ}$} & \textbf{$\mathbb{C}_{NEQ}$} & & & & & & & & \\
%   $\times$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & \textbf{87.04} & \textbf{93.5} & \textbf{88} & \textbf{99} \\
%   $\times$ & $\times$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & \uline{82.06} & \uline{91.0} & \textbf{88} & 94 \\
%   $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & 81.08 & 90.5 & 82 & \textbf{99} \\
%   $\times$ & $\circ$ & $\times$ & $\circ$ & $\circ$ & $\circ$ & 80.10 & 90.0 & \uline{84} & 96 \\
%   $\times$ & $\circ$ & $\circ$ & $\times$ & $\circ$ & $\circ$ & 79.09 & 89.5 & 82 & \uline{97} \\
%   $\times$ & $\circ$ & $\circ$ & $\circ$ & $\times$ & $\circ$ & 74.08 & 87.0 & 81 & 93 \\
%   $\times$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\times$ & 29.36 & 64.0 & 72 & 56
%   \end{tblr}
%   }
% \end{table}





% Exec denotes the execution results, Q denotes the question, KG denotes the external knowledge, C denotes the criteria, GT denotes the ground truth, and 

==> table/exp1/annotation_examples.tex <==


% False Positive
\begin{table}
\centering
\caption{False positive (instance \#49)}
\label{tab:tab_false_positive_real_example}
\adjustbox{max width=\columnwidth}{
% \begin{tblr}{
%   hline{1-2,4,6} = {1}{},
% }
% {\textbf{Q:~\textcolor[rgb]{0.192,0.2,0.247}{For the client whose loan was approved first in 1993/7/5, }}\\\textbf{\textcolor[rgb]{0.192,0.2,0.247}{what is the increase rate of his/her account balance\\from 1993/3/22 to 1998/12/27?}}} \\
% \textbf{Ground Truth (Considering multiple transactions in a day)}\\
% {SELECT CAST(
% \\~ (SUM(IIF(T3.date = '1998-12-27', T3.balance, 0)) -
% \\~ ~ SUM(IIF(T3.date = '1993-03-22', T3.balance, 0))) AS REAL)\\* 100 / SUM(IIF(T3.date = '1993-03-22', T3.balance, 0))
% \\FROM loan AS T1 INNER JOIN ACCOUNT AS T2\\ON T1.account\_id = T2.account\_id
% \\INNER JOIN trans AS T3 ON T3.account\_id = T2.account\_id
% \\WHERE T1.date = '1993-07-05'} \\
% \textbf{Prediction \textcolor{red}{(Limiting single transaction in a day)}} \\
% {SELECT CAST((t3.balance - t2.balance) * 100.0 / t2.balance AS REAL)
% \\FROM loan l INNER JOIN ACCOUNT a\\ON l.account\_id = a.account\_id
% \\INNER JOIN trans t2 ON t2.account\_id = a.account\_id \\ AND t2.date = '1993-03-22'
% \\INNER JOIN trans t3 ON t3.account\_id = a.account\_id \\ AND t3.date = '1998-12-27'
% \\WHERE l.date = '1993-07-05' LIMIT 1}                       
% \end{tblr}
\begin{tblr}{
  hline{1,6} = {1}{0.08em},
  hline{2,4} = {1}{},
}
{\textbf{Q: For the client whose loan was approved first in 1993/7/5, }\\\textbf{what is the increase rate of his/her account balance}\\\textbf{from 1993/3/22 to 1998/12/27?}}                                                                                                                                                                                     \\
\textbf{Ground Truth (Handling multiple transactions in a day)}                                                                                                                                                                                                                                                                                                     \\
{SELECT CAST(\\~ (SUM(IIF(T3.date = '1998-12-27', T3.balance, 0)) -\\~ ~ SUM(IIF(T3.date = '1993-03-22', T3.balance, 0))) AS REAL)\\~ 100 / SUM(IIF(T3.date = '1993-03-22', T3.balance, 0))\\FROM loan AS T1 INNER JOIN ACCOUNT AS T2\\ON T1.account\_id = T2.account\_id\\INNER JOIN trans AS T3 ON T3.account\_id = T2.account\_id\\WHERE T1.date = '1993-07-05'} \\
\textbf{Prediction \textcolor{red}{(Limiting single transaction in a day)}}                                                                                                                                                                                                                                                                                         \\
{SELECT CAST((t3.balance - t2.balance) * 100.0 \\~ / t2.balance AS REAL)\\FROM loan l INNER JOIN ACCOUNT a\\ON l.account\_id = a.account\_id\\INNER JOIN trans t2 ON t2.account\_id = a.account\_id \\ AND t2.date = '1993-03-22'\\INNER JOIN trans t3 ON t3.account\_id = a.account\_id \\ AND t3.date = '1998-12-27'\\WHERE l.date = '1993-07-05' \textbf{\textcolor{red}{LIMIT 1}}}        
\end{tblr}
}
\end{table}

% False Negative
% \usepackage{color}
% \usepackage{tabularray}
\begin{table}
\centering
\caption{False negative (instance \#26)}
\label{tab:tab_false_negative_real_example}
\adjustbox{max width=\columnwidth}{
\begin{tblr}{
  cell{2}{2} = {r=2}{},
  cell{4}{2} = {r=2}{},
  vline{2} = {-}{},
  vline{2} = {2}{-}{},
  hline{1,6} = {-}{0.08em},
  hline{2,4} = {-}{},
}
{\textbf{Q:~How many test takers are there at the schools }\\\textbf{whose mailing city address is in Fresno?}}                                                        & \textbf{Execution}                                                    \\
\textbf{Ground Truth}                                                                                                                                                  & { \textbar{} 5 \textbar{}\\\textbar{} 8 \textbar{}\\... \\(Sum 6070)} \\
{SELECT T1.NumTstTakr FROM satscores AS T1\\INNER JOIN schools AS T2 ON T1.cds = T2.CDSCode\\WHERE T2.MailCity = 'Fresno'}                                             &                                                                       \\
\textbf{Prediction}                                                                                                                                                    & 6070                                                                  \\
{SELECT \textbf{\textcolor{red}{SUM(satscores.NumTstTakr)}} FROM schools\\INNER JOIN satscores ON schools.CDSCode = satscores.cds\\WHERE schools.MailCity = 'Fresno';} &                                                                       
\end{tblr}
}

\end{table}

% True Positive



==> table/exp1/true_positive_v2.tex <==
\begin{table}[ht]
\caption{Noisy ground truth of BIRD (instance \#55). We simplified `enrollment (k-12)' + `enrollment (ages 5-17)' as Enrollment for readability.}
\resizebox{\columnwidth}{!}{%\
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{ll}
\hline
\textcolor{orange}{Question}           & \textit{List the codes of the schools } \\ 
                                       & \textit{with a total enrollment of over 500.} \\ \hdashline
\textcolor{blue}{Ground Truth}         & SELECT frpm.CDSCode FROM schools \\
                                       & \textcolor{blue}{INNER JOIN frpm} \\
                                       & \textcolor{blue}{ON schools.CDSCode = frpm.CDSCode} \\ 
                                       & WHERE Enrollment > 500 \\
                                       & \# Unnecessary table JOIN \\ \hdashline
\textcolor{Mint}{True Positive}        & SELECT cdscode FROM frpm \\
                                       & WHERE Enrollment > 500 \\ \hline

\end{tabular}}
\label{tab:tab_confusable_true_positive}
\end{table}


==> table/exp1/true_positives.tex <==

% \begin{table}
% \centering
% \caption{Confusable true positive (instance \#55)}

% \label{tab:tab_true_positive}
% \adjustbox{max width=\columnwidth}{
% \begin{tblr}{
%   hline{1-2,4,6} = {1}{},
% }
% \textbf{Q: List the codes of the schools with a total enrollment of over 500.}                                                                                                                                              \\
% \textbf{Ground Truth \textcolor{red}{(Unnecessary schools table JOIN)}}                                                                                                                                                     \\
% {SELECT T2.CDSCode \textcolor{red}{FROM schools AS T1} \textcolor{red}{}\\\textcolor{red}{INNER JOIN} frpm AS T2 ON T1.CDSCode = T2.CDSCode\\WHERE T2.\`{}Enrollment (K-12)\`{} + T2.\`{}Enrollment (Ages 5-17)\`{} \textgreater{} 500} \\
% \textbf{Prediction}                                                                                                                                                                                                         \\
% {SELECT cdscode~FROM frpm\\WHERE (\`{}enrollment (k-12)\`{} + \`{}enrollment (ages 5-17)\`{}) \textgreater{} 500}                                                                                                                       
% \end{tblr}
% }
% \end{table}


\begin{figure}[h]
\centering
\begin{defin}
Q: List the codes of the schools with a total enrollment of over 500.

\begin{lstlisting}[
  style=SQL,
  title=Ground Truth Query
]
SELECT frpm.CDSCode FROM schools INNER JOIN frpm
ON schools.CDSCode = frpm.CDSCode
WHERE Enrollment > 500
# Unnecessary table JOIN
\end{lstlisting}

\begin{lstlisting}[style=SQL, title=Generated Query (True Positive)]
SELECT cdscode FROM frpm 
WHERE Enrollment > 500
\end{lstlisting}
\end{defin}

\caption{Confusable true positive (instance \#55). We simplified \`{}enrollment (k-12)\`{} + \`{}enrollment (ages 5-17)\`{} as Enrollment for readability.}
\label{fig:fig_confusable_true_positive}
\end{figure}





==> table/exp2/error_analysis_bird.tex <==
\begin{table*}[]
\centering
\caption{BIRD false negatives}
\label{tab:tab_fn_bird}
\adjustbox{max width=\linewidth}{
\begin{tabular}{llllll}
\toprule
model & Structure & Value Repr. & Ground Truth & Multiple Answers & Other \\
\midrule
C3\_SQL & 79 (63.20\%) & 11 (8.80\%) & 56 (44.80\%) & 10 (8.00\%) & 14 (11.20\%) \\
CHESS-GPT-4o-mini & 77 (53.85\%) & 14 (9.79\%) & 84 (58.74\%) & 17 (11.89\%) & 18 (12.59\%) \\
DAIL\_SQL\_9-SHOT\_MP & 93 (60.39\%) & 21 (13.64\%) & 81 (52.60\%) & 15 (9.74\%) & 17 (11.04\%) \\
DAIL\_SQL\_9-SHOT\_QM & 92 (60.53\%) & 23 (15.13\%) & 82 (53.95\%) & 7 (4.61\%) & 17 (11.18\%) \\
DTS-SQL-BIRD-GPT4o-0823 & 58 (54.21\%) & 14 (13.08\%) & 70 (65.42\%) & 10 (9.35\%) & 11 (10.28\%) \\
SFT\_CodeS\_15B\_EK & 50 (56.18\%) & 15 (16.85\%) & 50 (56.18\%) & 6 (6.74\%) & 10 (11.24\%) \\
SFT\_CodeS\_3B\_EK & 41 (56.94\%) & 9 (12.50\%) & 37 (51.39\%) & 4 (5.56\%) & 10 (13.89\%) \\
SFT\_CodeS\_7B\_EK & 41 (62.12\%) & 10 (15.15\%) & 32 (48.48\%) & 4 (6.06\%) & 8 (12.12\%) \\
SuperSQL & 104 (63.41\%) & 24 (14.63\%) & 83 (50.61\%) & 11 (6.71\%) & 22 (13.41\%) \\
TA-ACL & 80 (57.55\%) & 18 (12.95\%) & 75 (53.96\%) & 8 (5.76\%) & 16 (11.51\%) \\
\midrule
\textbf{Average} & 71 (58.84\%) & 15 (13.25\%) & 65 (53.61\%) & 9 (7.44\%) & 14 (11.85\%) \\
\bottomrule
\end{tabular}
}
\end{table*}


\begin{table*}[]
\centering
\caption{BIRD false positives}
\label{tab:tab_fp_bird}
\adjustbox{max width=\linewidth}{
\begin{tabular}{lllllll}
\toprule
model & Schema Link. & Filtering Cond. & Nullable Col. & Multiple Rows & Abused Clauses & Other \\
\midrule
C3\_SQL & 19 (31.15\%) & 35 (57.38\%) & 1 (1.64\%) & 14 (22.95\%) & 10 (16.39\%) & 8 (13.11\%) \\
CHESS-GPT-4o-mini & 23 (34.33\%) & 28 (41.79\%) & 1 (1.49\%) & 18 (26.87\%) & 7 (10.45\%) & 14 (20.90\%) \\
DAIL\_SQL\_9-SHOT\_MP & 14 (29.17\%) & 19 (39.58\%) & 3 (6.25\%) & 12 (25.00\%) & 5 (10.42\%) & 7 (14.58\%) \\
DAIL\_SQL\_9-SHOT\_QM & 13 (24.07\%) & 23 (42.59\%) & 1 (1.85\%) & 21 (38.89\%) & 6 (11.11\%) & 7 (12.96\%) \\
DTS-SQL-BIRD-GPT4o-0823 & 30 (37.97\%) & 33 (41.77\%) & 6 (7.59\%) & 26 (32.91\%) & 7 (8.86\%) & 9 (11.39\%) \\
SFT\_CodeS\_15B\_EK & 15 (22.06\%) & 36 (52.94\%) & 1 (1.47\%) & 25 (36.76\%) & 8 (11.76\%) & 6 (8.82\%) \\
SFT\_CodeS\_3B\_EK & 19 (29.69\%) & 35 (54.69\%) & 2 (3.12\%) & 19 (29.69\%) & 6 (9.38\%) & 6 (9.38\%) \\
SFT\_CodeS\_7B\_EK & 19 (23.17\%) & 44 (53.66\%) & 4 (4.88\%) & 30 (36.59\%) & 8 (9.76\%) & 10 (12.20\%) \\
SuperSQL & 19 (34.55\%) & 21 (38.18\%) & 3 (5.45\%) & 17 (30.91\%) & 5 (9.09\%) & 10 (18.18\%) \\
TA-ACL & 7 (14.00\%) & 30 (60.00\%) & 1 (2.00\%) & 18 (36.00\%) & 8 (16.00\%) & 6 (12.00\%) \\
\midrule
\textbf{Average} & 17 (28.02\%) & 30 (48.26\%) & 2 (3.58\%) & 20 (31.66\%) & 7 (11.32\%) & 8 (13.35\%) \\
\bottomrule
\end{tabular}
}
\end{table*}




\begin{table*}[]
\centering
\caption{BIRD true negatives}
\label{tab:tab_tn_bird}
\adjustbox{max width=\linewidth}{
\begin{tabular}{llllllll}
\toprule
model & Error & Schema Link. & Filtering Cond. & Nullable Col. & Multiple Rows & Abused Clauses & Other \\
\midrule
C3\_SQL & 17 (2.55\%) & 249 (37.39\%) & 363 (54.50\%) & 18 (2.70\%) & 197 (29.58\%) & 112 (16.82\%) & 180 (27.03\%) \\
CHESS-GPT-4o-mini & 21 (4.34\%) & 226 (46.69\%) & 173 (35.74\%) & 13 (2.69\%) & 140 (28.93\%) & 44 (9.09\%) & 114 (23.55\%) \\
DAIL\_SQL\_9-SHOT\_MP & 96 (17.17\%) & 158 (28.26\%) & 277 (49.55\%) & 18 (3.22\%) & 130 (23.26\%) & 49 (8.77\%) & 83 (14.85\%) \\
DAIL\_SQL\_9-SHOT\_QM & 97 (17.08\%) & 159 (27.99\%) & 284 (50.00\%) & 27 (4.75\%) & 127 (22.36\%) & 52 (9.15\%) & 100 (17.61\%) \\
DTS-SQL-BIRD-GPT4o-0823 & 60 (11.19\%) & 204 (38.06\%) & 268 (50.00\%) & 23 (4.29\%) & 139 (25.93\%) & 40 (7.46\%) & 93 (17.35\%) \\
SFT\_CodeS\_15B\_EK & 9 (1.56\%) & 195 (33.74\%) & 344 (59.52\%) & 25 (4.33\%) & 170 (29.41\%) & 65 (11.25\%) & 118 (20.42\%) \\
SFT\_CodeS\_3B\_EK & 28 (4.36\%) & 230 (35.83\%) & 367 (57.17\%) & 21 (3.27\%) & 184 (28.66\%) & 93 (14.49\%) & 130 (20.25\%) \\
SFT\_CodeS\_7B\_EK & 19 (3.04\%) & 226 (36.10\%) & 350 (55.91\%) & 24 (3.83\%) & 187 (29.87\%) & 64 (10.22\%) & 127 (20.29\%) \\
SuperSQL & 23 (4.69\%) & 172 (35.10\%) & 252 (51.43\%) & 23 (4.69\%) & 143 (29.18\%) & 63 (12.86\%) & 99 (20.20\%) \\
TA-ACL & 125 (23.11\%) & 125 (23.11\%) & 222 (41.04\%) & 17 (3.14\%) & 125 (23.11\%) & 52 (9.61\%) & 99 (18.30\%) \\
\midrule
\textbf{Average} & 49 (8.91\%) & 194 (34.23\%) & 290 (50.49\%) & 20 (3.69\%) & 154 (27.03\%) & 63 (10.97\%) & 114 (19.98\%) \\
\bottomrule
\end{tabular}
}
\end{table*}


==> table/exp2/error_analysis_spider.tex <==
\begin{table*}[]
\centering
\caption{False negatives of the top ten Spider models}
\label{tab:tab_fn_spider}
\adjustbox{max width=\linewidth}{
\begin{tabular}{llllll}
\toprule
Model & Structure & Value Repr. & Ground Truth & Multiple Answers & Other \\
\midrule
C3\_SQL & 44 (55.00\%) & 7 (8.75\%) & 32 (40.00\%) & 6 (7.50\%) & 17 (21.25\%) \\
DAILSQL & 35 (44.87\%) & 7 (8.97\%) & 39 (50.00\%) & 8 (10.26\%) & 7 (8.97\%) \\
DAILSQL\_SC & 30 (40.54\%) & 7 (9.46\%) & 32 (43.24\%) & 7 (9.46\%) & 8 (10.81\%) \\
DINSQL & 42 (43.30\%) & 8 (8.25\%) & 43 (44.33\%) & 15 (15.46\%) & 12 (12.37\%) \\
SFT\_CodeS\_15B & 15 (35.71\%) & 2 (4.76\%) & 22 (52.38\%) & 6 (14.29\%) & 6 (14.29\%) \\
SFT\_CodeS\_3B & 16 (42.11\%) & 4 (10.53\%) & 15 (39.47\%) & 1 (2.63\%) & 6 (15.79\%) \\
SFT\_CodeS\_7B & 14 (37.84\%) & 1 (2.70\%) & 18 (48.65\%) & 1 (2.70\%) & 5 (13.51\%) \\
SFT\_Deepseek\_Coder\_7B & 21 (37.50\%) & 2 (3.57\%) & 23 (41.07\%) & 5 (8.93\%) & 16 (28.57\%) \\
SuperSQL & 27 (48.21\%) & 8 (14.29\%) & 25 (44.64\%) & 5 (8.93\%) & 9 (16.07\%) \\
TA-ACL & 32 (54.24\%) & 3 (5.08\%) & 28 (47.46\%) & 5 (8.47\%) & 8 (13.56\%) \\
\midrule
Average & 27 (43.93\%) & 4 (7.64\%) & 27 (45.12\%) & 5 (8.86\%) & 9 (15.52\%) \\
\bottomrule
\end{tabular}
}


\end{table*}
\begin{table*}[]
\centering
\caption{False positives of the top ten Spider models}
\label{tab:tab_fn_spider}
\adjustbox{max width=\linewidth}{
\begin{tabular}{lllllll}
\toprule
Model & Schema Linking & Filtering Condition & Nullable Column & Multiple Rows & Abused Clauses & Other \\
\midrule
C3\_SQL & 8 (47.06\%) & 11 (64.71\%) & 0 (0.00\%) & 2 (11.76\%) & 4 (23.53\%) & 0 (0.00\%) \\
DAILSQL & 7 (43.75\%) & 7 (43.75\%) & 0 (0.00\%) & 5 (31.25\%) & 4 (25.00\%) & 0 (0.00\%) \\
DAILSQL\_SC & 7 (58.33\%) & 7 (58.33\%) & 0 (0.00\%) & 2 (16.67\%) & 0 (0.00\%) & 0 (0.00\%) \\
DINSQL & 10 (62.50\%) & 3 (18.75\%) & 1 (6.25\%) & 2 (12.50\%) & 3 (18.75\%) & 0 (0.00\%) \\
SFT\_CodeS\_15B & 8 (50.00\%) & 7 (43.75\%) & 0 (0.00\%) & 4 (25.00\%) & 3 (18.75\%) & 2 (12.50\%) \\
SFT\_CodeS\_3B & 8 (42.11\%) & 8 (42.11\%) & 0 (0.00\%) & 8 (42.11\%) & 1 (5.26\%) & 3 (15.79\%) \\
SFT\_CodeS\_7B & 11 (64.71\%) & 9 (52.94\%) & 0 (0.00\%) & 2 (11.76\%) & 2 (11.76\%) & 1 (5.88\%) \\
SFT\_Deepseek\_Coder\_7B & 4 (30.77\%) & 8 (61.54\%) & 0 (0.00\%) & 2 (15.38\%) & 0 (0.00\%) & 2 (15.38\%) \\
SuperSQL & 8 (61.54\%) & 1 (7.69\%) & 0 (0.00\%) & 6 (46.15\%) & 2 (15.38\%) & 0 (0.00\%) \\
TA-ACL & 11 (61.11\%) & 8 (44.44\%) & 0 (0.00\%) & 5 (27.78\%) & 1 (5.56\%) & 0 (0.00\%) \\
\midrule
Average & 8 (52.19\%) & 6 (43.80\%) & 0 (0.62\%) & 3 (24.04\%) & 2 (12.40\%) & 0 (4.96\%) \\
\bottomrule
\end{tabular}
}
\end{table*}

\begin{table*}[]
\centering
\caption{True negatives of the top ten Spider models}
\label{tab:tab_fn_spider}
\adjustbox{max width=\linewidth}{
\begin{tabular}{llllllll}
\toprule
Model & Error & Schema Linking & Filtering Condition & Nullable Column & Multiple Rows & Abused Clauses & Other \\
\midrule
C3\_SQL & 1 (0.94\%) & 35 (33.02\%) & 67 (63.21\%) & 0 (0.00\%) & 21 (19.81\%) & 19 (17.92\%) & 11 (10.38\%) \\
DAILSQL & 14 (14.43\%) & 16 (16.49\%) & 61 (62.89\%) & 1 (1.03\%) & 16 (16.49\%) & 5 (5.15\%) & 8 (8.25\%) \\
DAILSQL\_SC & 0 (0.00\%) & 30 (31.25\%) & 56 (58.33\%) & 1 (1.04\%) & 21 (21.88\%) & 7 (7.29\%) & 10 (10.42\%) \\
DINSQL & 10 (12.35\%) & 16 (19.75\%) & 51 (62.96\%) & 0 (0.00\%) & 17 (20.99\%) & 10 (12.35\%) & 4 (4.94\%) \\
SFT\_CodeS\_15B & 4 (3.51\%) & 33 (28.95\%) & 66 (57.89\%) & 0 (0.00\%) & 29 (25.44\%) & 17 (14.91\%) & 9 (7.89\%) \\
SFT\_CodeS\_3B & 5 (3.70\%) & 36 (26.67\%) & 76 (56.30\%) & 0 (0.00\%) & 30 (22.22\%) & 35 (25.93\%) & 13 (9.63\%) \\
SFT\_CodeS\_7B & 5 (4.39\%) & 28 (24.56\%) & 67 (58.77\%) & 0 (0.00\%) & 30 (26.32\%) & 19 (16.67\%) & 12 (10.53\%) \\
SFT\_Deepseek\_Coder\_7B & 39 (27.27\%) & 42 (29.37\%) & 62 (43.36\%) & 0 (0.00\%) & 16 (11.19\%) & 12 (8.39\%) & 10 (6.99\%) \\
SuperSQL & 0 (0.00\%) & 17 (21.79\%) & 50 (64.10\%) & 0 (0.00\%) & 19 (24.36\%) & 9 (11.54\%) & 8 (10.26\%) \\
TA-ACL & 8 (8.33\%) & 23 (23.96\%) & 48 (50.00\%) & 0 (0.00\%) & 26 (27.08\%) & 6 (6.25\%) & 16 (16.67\%) \\
\midrule
Average & 8 (7.49\%) & 27 (25.58\%) & 60 (57.78\%) & 0 (0.21\%) & 22 (21.58\%) & 13 (12.64\%) & 10 (9.59\%) \\
\bottomrule
\end{tabular}
}
\end{table*}

==> table/exp2/hardness_result.tex <==
\begin{table*}[]
\centering
\caption{Spider-dev result}
\label{tab:tab_hardness_spider}
\begin{tabular}{llllll}
\toprule
\textbf{hardness} & \textbf{EX} & \textbf{FLEX} & \textbf{FLEX - EX} & \textbf{FPR} & \textbf{FNR} \\
\midrule
easy & 88.08 ± 10.60 & 89.64 ± 8.66 & 1.56 ± 3.08 & 1.38 ± 0.94 & 2.94 ± 3.03 \\
medium & 78.93 ± 15.01 & 79.58 ± 15.02 & 0.65 ± 2.97 & 3.05 ± 1.54 & 3.70 ± 2.66 \\
hard & 64.14 ± 16.40 & 67.30 ± 16.79 & 3.16 ± 5.25 & 3.47 ± 1.79 & 6.63 ± 4.76 \\
extra & 49.74 ± 16.50 & 57.93 ± 19.69 & 8.19 ± 7.07 & 3.92 ± 1.87 & 12.11 ± 6.32 \\
\bottomrule
\end{tabular}
\end{table*}


\begin{table*}[]
\centering
\caption{BIRD-dev result}
\label{tab:tab_hardness_bird}
\begin{tabular}{llllll}
\toprule
\textbf{hardness} & \textbf{EX} & \textbf{FLEX} & \textbf{FLEX - EX} & \textbf{FPR} & \textbf{FNR} \\
\midrule
simple & 55.79 ± 9.36 & 59.95 ± 10.16 & 4.15 ± 3.04 & 2.61 ± 0.95 & 6.76 ± 2.38 \\
moderate & 35.51 ± 10.85 & 39.64 ± 12.30 & 4.14 ± 3.99 & 4.20 ± 1.53 & 8.34 ± 3.71 \\
challenging & 32.24 ± 11.15 & 29.66 ± 11.58 & -2.59 ± 2.92 & 8.14 ± 2.12 & 5.55 ± 2.88 \\
\bottomrule
\end{tabular}
\end{table*}


==> table/intro/spider_flex_leaderboard.tex <==

\begin{table}[!t]
\centering
\caption{Spider dev set top 10 leaderboard re-ranked by \ours. $\Delta$ denotes FLEX $-$ EX}
\label{tab:tab_intro_spider}
\adjustbox{max width=\columnwidth}{
\begin{tabular}{llccc}
\toprule
\textbf{Rank} & \textbf{Model} & \textbf{FLEX} & \textbf{EX} & \textbf{$\Delta$} \\
\midrule
\phantom{0}1\phantom{0}(-) & SuperSQL & \textbf{91.20} & \textbf{87.04} & $+4.16$ \\
\phantom{0}2\phantom{0}(\textcolor{red}{↑7}) & DINSQL & 90.62 & 82.79 & $+7.83$ \\
\phantom{0}3\phantom{0}(\textcolor{red}{↑3}) & DAILSQL\_SC & 89.56 & 83.56 & $+6.00$ \\
\phantom{0}4\phantom{0}(\textcolor{red}{↑4}) & DAILSQL & 89.07 & 83.08 & $+6.00$ \\
\phantom{0}5\phantom{0}(\textcolor{blue}{↓2}) & TA-ACL & 88.97 & 85.01 & $+3.97$ \\
\phantom{0}6\phantom{0}(\textcolor{red}{↑4}) & C3\_SQL & 88.10 & 82.01 & $+6.09$ \\
\phantom{0}7\phantom{0}(\textcolor{blue}{↓3}) & SFT\_CodeS\_15B & 87.43 & 84.91 & $+2.51$ \\
\phantom{0}8\phantom{0}(\textcolor{blue}{↓6}) & SFT\_CodeS\_7B & 87.33 & 85.40 & $+1.93$ \\
\phantom{0}9\phantom{0}(\textcolor{blue}{↓2}) & SFT\_CodeS\_3B & 85.11 & 83.27 & $+1.84$ \\
10\phantom{0}(\textcolor{red}{↑4}) & SFT\_Deepseek\_Coder\_7B & 84.91 & 80.75 & $+4.16$ \\
\bottomrule
\end{tabular}
}
\end{table}

==> table/method/baseline_comparison.tex <==
\begin{table*}
\centering
\caption{Baselines}
\label{tab:tab_method_baselines}
\adjustbox{max width=\textwidth}{
\begin{tblr}{
  vline{2} = {-}{},
  hline{1,4} = {-}{0.08em},
  hline{2} = {-}{},
}
\textbf{Method}         & \textbf{Target Metric} & \textbf{FP/FN Analysis} & \textbf{Fine-grained Metrics} & \textbf{Revaluated Benchmark (#*)} \\
LLM-SQL-Solver~\cite{zhao2024llmsqlsolverllmsdeterminesql}          & EX                     & \xmark                       & \xmark                                 & Spider
  (3)                         \\
\textbf{LLM-as-a-Judge (ours)} & Human                  & \checkmark                     & \checkmark                               & Spider
  (10+), BIRD (10+)           
\end{tblr}
}
\end{table*}

==> table/method/llm_judge_eval.tex <==
% \usepackage{tabularray}
\begin{table}[!t]
\centering
\caption{Agreement between LLM judgments and human consensus. Kappa denotes Cohen's kappa score, Acc denotes accuracy score. The higher score is better.}
\label{tab:tab_llm_human_agreement}
\adjustbox{max width=\columnwidth}{
\begin{tblr}{
  row{3} = {c},
  row{13} = {c},
  column{2} = {c},
  column{3} = {c},
  cell{3}{1} = {c=3}{},
  cell{13}{1} = {c=3}{},
  hline{1,31} = {-}{0.08em},
  hline{2} = {-}{},
  hline{3-4,13-14} = {-}{dotted},
}
\textbf{Model}                     & \textbf{Kappa} & \textbf{Acc}   \\
EX                                 & 62.00          & 81.00          \\
\ours \textit{w/ Proprietary LMs } &                &                \\
GPT-4o-2024-08-06                  & \textbf{87.04} & \textbf{93.50} \\
GPT-4o-mini-2024-07-18             & 61.54          & 81.00          \\
GPT-4-turbo-2024-04-09             & 60.66          & 80.00          \\
GPT-4-0125-Preview                 & 54.78          & 77.00          \\
GPT-3.5-turbo-0125                 & 53.69          & 76.50          \\
Claude-3-5-sonnet-20240620         & \uline{80.02}  & \uline{90.00}  \\
Claude-3-haiku-20240307            & 49.90          & 74.50          \\
Gemini-1.5-pro                     & 77.06          & 88.50          \\
Gemini-1.5-flash                   & 68.96          & 84.50          \\
\ours \textit{w/ Open LMs }        &                &                \\
DeepSeek-Coder-V2-Instruct-0724    & 76.13          & 88.00          \\
DeepSeek-V2-Chat                   & 77.14          & 88.50          \\
DeepSeek-Coder-V2-Lite-Instruct    & 51.25          & 75.00          \\
DeepSeek-V2-Lite-Chat              & 49.98          & 74.50          \\
Deepseek-Coder-7B-Instruct-v1.5    & 17.43          & 57.00          \\
Mistral-Large-Instruct-2407        & 77.03          & 88.50          \\
Mixtral-8x7B-Instruct-v0.1         & 50.04          & 72.50          \\
Mistral-Small-Instruct-2409        & 79.03          & 89.50          \\
Mistral-7B-Instruct-v0.3           & 53.58          & 76.50          \\
Llama-3.1-70B-Instruct             & 72.09          & 86.00          \\
Llama-3.1-8B-Instruct              & 69.18          & 84.50          \\
Qwen2.5-72B-Instruct               & 74.10          & 87.00          \\
Qwen2.5-Coder-7B-Instruct          & 64.96          & 82.50          \\
Qwen2.5-7B-Instruct                & 58.07          & 79.00          \\
Gemma-2-27b-it                     & 67.00          & 81.00          \\
Gemma-2-9b-it                      & 66.12          & 83.00          \\
EXAONE-3.0-7.8B-Instruct           & 47.81          & 73.50          
\end{tblr}
}
\end{table}



==> table/pre/error-column-mismatch.tex <==
% \usepackage{tabularray}
\begin{table}
\centering
\caption{False negative example 1: Different output structures}
\label{tab:tab_column_mismatch}
\adjustbox{max width=\columnwidth}{
\begin{tblr}{
  vline{2} = {-}{},
  hline{1,6} = {-}{0.08em},
  hline{2} = {-}{},
}
\textbf{Question}        & What are the grades of all students?         \\
\textbf{GT Query}        & SELECT \textbf{name, score}~FROM student     \\
\textbf{Overused Column} & SELECT \textbf{id, name, score}~FROM student \\
\textbf{Missed Column}   & SELECT \textbf{score}~FROM student           \\
\textbf{Order Mismatch}  & SELECT \textbf{score, name} FROM student     
\end{tblr}
}
\end{table}

==> table/pre/error-multirow.tex <==
\begin{table}
\centering
\caption{The self-refine prompt utilized in our study}
\label{tab:tab_refine_prompt}
\begin{tblr}{
  hline{1,4} = {-}{0.08em},
}
\textbf{Question}                                                                    & What is the \textbf{average writing score }of each of the schools managed by Ricci Ulrich? List the schools and the corresponding average writing scores.                                                                                                   \\
{\textbf{GT Query}\\\textbf{ }\textcolor[rgb]{0.082,0.376,0.51}{\textbf{(Correct)}}} & {SELECT T2.School, \textcolor[rgb]{0.082,0.376,0.51}{\textbf{T1.AvgScrWrite}} FROM satscores AS T1\\INNER
  JOIN schools AS T2 ON T1.cds = T2.CDSCode
  \\WHERE
  T2.AdmFName1 = 'Ricci'
  AND
  T2.AdmLName1 = 'Ulrich'
  }                                \\
{\textbf{Generated Query}\\\textcolor{red}{\textbf{(Incorrect)}}}                    & {SELECT T1.sname, \textcolor{red}{\textbf{AVG(T1.avgscrwrite)}} FROM satscores AS T1\\INNER
  JOIN schools AS T2 ON T1.cds = T2.cdscode
  \\WHERE
  T2.admfname1 = 'Ricci'
  AND
  T2.admlname1 = 'Ulrich'
  \\\textcolor{red}{\textbf{GROUP BY T1.sname}}} 
\end{tblr}
\end{table}

==> table/pre/error-value-misrep.tex <==

\begin{table*}[t]
\centering
\caption{False negative example 2: Output representation differs due to the ambiguous question. The {\`{}Percent(\%) Eligible FRPM (Ages 5-17)\`{}} in the question can be interpreted to the column of the same name, which has the result of {\`{}FRPM Count(Ages 5-17)\`{}  / \`{}Enrollment (Ages 5-17)\`{}}, but range from 0 to 1.}
\label{tab:tab_mispresented_value}
\adjustbox{max width=\textwidth}{%

\begin{tblr}{
  vline{2-3} = {-}{},
  vline{3} = {2}{-}{},
  hline{1,4} = {-}{0.08em},
  hline{2} = {-}{},
}
\textbf{Question}     & What are the \textbf{Percent (\%) Eligible FRPM (Ages 5-17) }of the schools?                   & \textbf{Execution Result}  \\
\textbf{Ground Truth} & SELECT \`{}\textbf{FRPM Count(Ages 5-17)\`{} * 100 / \`{}Enrollment (Ages 5-17)\`{}~}FROM frpm & \textbf{\textbf{3.7558}}   \\
\textbf{Prediction}   & SELECT \`{}\textcolor{red}{\textbf{Percent(\%) Eligible FRPM (Ages 5-17)\`{}}}~FROM frpm       & \textbf{\textbf{0.037558}} 
\end{tblr}
}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[t]
% \centering
% \caption{False negative example 2: misrepresented value}
% \label{tab:tab_mispresented_value}
% \adjustbox{max width=\columnwidth}{%
% \begin{tblr}{
%   hline{1,6} = {1}{0.08em},
%   hline{2,4} = {1}{},
% }
% {Questions: Which schools served a grade span
% of Kindergarten to 9th grade in the county \\of Los Angeles and \textbf{whatis its Percent (\%) Eligible FRPM (Ages 5-17)?}}                                                                                                                                                                                                                                 \\
% \textbf{GT Query}                                                                                                                                                                                                                                                                                                                                                                                          \\
% {SELECT T2.School, T1.\`{}FRPM Count
% (Ages 5-17)\`{} * 100 / T1.\`{}Enrollment (Ages 5-17)\`{}
% \\FROM frpm AS T1 INNER JOIN schools AS T2 ON
% T1.CDSCode = T2.CDSCode
% \\WHERE T2.County = 'Los Angeles’ AND
% T2.GSserved = 'K-9’
% \\
% --Result--\\
% \textbar{} White Oak Elementary \textbar{} \textbf{3.755868544600939} \textbar{}\\
% \textbar{} The Accelerated \textbar{} \textbf{97.63888888888889} \textbar{}}           \\
% {\textbf{Generated Query} \textcolor{red}{\textbf{(Different Result)}}}                                                                                                                                                                                                                                                                                                                       \\
% {SELECT schools.School, \textcolor{red}{\textbf{frpm.\`{}Percent(\%) Eligible FRPM (Ages 5-17)\`{}}}\\FROM schools INNER JOIN frpm ON schools.CDSCode =
% frpm.CDSCode
% \\WHERE schools.GSserved = 'K-9’ AND
% schools.County = 'Los Angeles’;\\
% --Result--
% \\\textbar{} White Oak Elementary \textbar{} \textbf{0.0375586854460094} \textbar{}\\\textbar{} The Accelerated \textbar{} \textbf{0.976388888888889} \textbar{}} 
% \end{tblr}
% }
% \end{table}

==> table/pre/simple_error_cases.tex <==

\begin{figure}[h]
\centering
\begin{defin}
Q: Who has the highest score?

\begin{lstlisting}[style=SQL, title=Ground Truth Query]
SELECT name FROM student
ORDER BY score DESC LIMIT 1
> John
\end{lstlisting}

\begin{lstlisting}[style=SQL, title=False Negative 1]
SELECT name, score FROM student
ORDER BY score LIMIT 1
> John, 90
\end{lstlisting}

\begin{lstlisting}[style=SQL, title=False Negative 2]
SELECT name FROM student
WHERE score == MAX(score)
> John, Smith 
# Two students have the highest score.
\end{lstlisting}

\begin{lstlisting}[style=SQL, title=False Positive 1]
SELECT name FROM student
WHERE age < 19
ORDER BY score DESC LIMIT 1
> John
# Unnecessary condition
\end{lstlisting}
\end{defin}
\caption{Examples of false negative and false positive}
\label{fig:fig_fp_fn_example}
\end{figure}
% \begin{figure}[!ht]
% \centering
% \resizebox{0.5\textwidth}{!}{%
% \begin{circuitikz}
% \tikzstyle{every node}=[font=\LARGE]

% \node (tikzmaker) [shift={(0, --0.25)}] at (8,7.75) {\includegraphics[width=0cm]{}};
% \node (tikzmaker) [shift={(1, -0)}] at (6.5,12.75) {\includegraphics[width=2cm]{}};
% \node (tikzmaker) [shift={(1, -0)}] at (5.5,11.25) {\includegraphics[width=2cm]{}};
% \node [font=\normalsize] at (18,4.25) {SELECT name FROM student ORDER BY score DESC LIMIT 1 > John};
% \node (tikzmaker) [shift={(1, -0)}] at (15,9.25) {\includegraphics[width=2cm]{}};
% \node (tikzmaker) [shift={(1, -0)}] at (15,9.75) {\includegraphics[width=2cm]{}};
% \node (tikzmaker) [shift={(1, -0)}] at (18,10.75) {\includegraphics[width=2cm]{png}};
% \node (tikzmaker) [shift={(1, -0)}] at (18,10.75) {\includegraphics[width=2cm]{png}};
% \node (tikzmaker) [shift={(1, -0)}] at (18,9.75) {\includegraphics[width=2cm]{png}};
% \node (tikzmaker) [shift={(1, -0)}] at (18,6.25) {\includegraphics[width=2cm]{png}};
% \node (tikzmaker) [shift={(1, -0)}] at (16,5.25) {\includegraphics[width=2cm]{png}};



% \node (tikzmaker) [shift={(1, -0)}] at (16,9.25) {\includegraphics[width=2cm]{}};
% \node (tikzmaker) [shift={(1, -0)}] at (16,9.75) {\includegraphics[width=2cm]{}};
% \node (tikzmaker) [shift={(1, -0)}] at (15.5,10.25) {\includegraphics[width=2cm]{}};
% \node (tikzmaker) [shift={(1, -0)}] at (15.5,9.75) {\includegraphics[width=2cm]{}};
% \node [font=\normalsize] at (14.5,5.5) {Ground Truth Query};


% \node [font=\normalsize] at (13.5,8) {Question};
% \node [font=\normalsize] at (15,6.75) {Who has the highest score?};
% \draw [ rounded corners = 14.4] (12.5,8.75) rectangle (23.75,7.5);
% \draw [ rounded corners = 14.4] (12.5,8.75) rectangle (23.75,2.5);
% \draw [ rounded corners = 14.4] (12.5,6.25) rectangle (23.75,5);
% \end{circuitikz}
% }%

% \label{fig:my_label}
% \end{figure}

==> table/pre/strict_errors.tex <==


\begin{table}[t]
\centering
\caption{False positive example 1: Incorrect filtering condition in the WHERE clause.}
\label{tab:strict_error_incorrect_logic}
\adjustbox{max width=\columnwidth}{
\begin{tblr}{
  hlines,
  hline{1,6} = {1}{0.08em},
}
\textbf{Q:} What type of bond is there between the
atoms TR004\_8 and TR004\_20?~ ~ ~~                                                                                                                                                                                                                                                                                      \\
\textbf{Ground Truth Query}                                                                                                                                                                                                                                                                                                                                        \\
{SELECT T1.bond\_type FROM bond AS T1
\\INNER JOIN connected AS T2 ON T1.bond\_id
= T2.bond\_id
\\WHERE \textbf{T2.atom\_id = 'TR004\_8’ AND T2.atom\_id2 = 'TR004\_20}\textbf{'}\textcolor[rgb]{0.082,0.376,0.51}\\{\textbf{~ ~ OR T2.atom\_id2 = 'TR004\_8’AND T2.atom\_id = 'TR004\_20'}}} \\
\textbf{Prediction Query (Incorrect but result is same)}                                                                                                                                                                                                                                                                                                                                          \\
{SELECT bond.bond\_type FROM
connected
\\JOIN bond ON connected.bond\_id = bond.bond\_id
\\~WHERE \textcolor{red}{\textbf{connected.atom\_id}}\textcolor{red}{\textbf{= 'TR004\_8’ }}\\\textcolor{red}{\textbf{~~~ AND connected.atom\_id2 = 'TR004\_20'}}}                                                                                                        
\end{tblr}
}
\end{table}

\begin{table}[t]
\centering

\caption{False positive example 2: The school column is not unique, and there could be schools with the same name.}
\label{tab:strict_error_assuming_not_unique}
\adjustbox{max width=\columnwidth}{
\begin{tblr}{
  hlines,
  hline{1,6} = {1}{0.08em},
}
\textbf{Q: }What is the \textbf{average writing score }of each of the schools~ ~ ~                                                                                                    \\
\textbf{Ground Truth Query}                                                                                                                                                        \\
{SELECT T2.School, \textcolor[rgb]{0.082,0.376,0.51}{\textbf{T1.AvgScrWrite}} FROM satscores AS T1\\INNER JOIN schools AS T2 ON T1.cds =T2.CDSCode~ ~ ~~}                            \\
\textbf{Prediction Query (Incorrect but result is same)}                                                                                                                                                          \\
{SELECT T1.sname, \textcolor{red}{\textbf{AVG(T1.avgscrwrite)}} FROM satscores AS T1\\INNER JOIN schools AS T2 ON T1.cds =
T2.cdscode\\\textcolor{red}{\textbf{GROUP BY T1.sname}}} 
\end{tblr}
}
\end{table}
